Emerging from Ground: Addressing Intent Deviation in Tool-Using Agents via Deriving Real Calls into Virtual Trajectories

LLMs have advanced tool-using agents for real-world applications, yet they often lead to unexpected behaviors or results. Beyond obvious failures, the subtle issue of "intent deviation" severely hinders reliable evaluation and performance improvement. Existing post-training methods generally leverage either real system samples or virtual data simulated by LLMs. However, the former is costly due to reliance on hand-crafted user requests, while the latter suffers from distribution shift from the real tools in the wild. Additionally, both methods lack negative samples tailored to intent deviation scenarios, hindering effective guidance on preference learning. We introduce RISE, a "Real-to-Virtual" method designed to mitigate intent deviation. Anchoring on verified tool primitives, RISE synthesizes virtual trajectories and generates diverse negative samples through mutation on critical parameters. With synthetic data, RISE fine-tunes backbone LLMs via the two-stage training for intent alignment. Evaluation results demonstrate that data synthesized by RISE achieve promising results in eight metrics covering user requires, execution trajectories and agent responses. Integrating with training, RISE achieves an average 35.28% improvement in Acctask (task completion) and 23.27% in Accintent (intent alignment), outperforming SOTA baselines by 1.20--42.09% and 1.17--54.93% respectively.

==> section/backup/result_20260115.tex <==
\section{Results}
\subsection{Results of Data Quality (RQ1)}
% \yang{comment.}
%RQ1这块文字表述还是有点不清楚，你按照如下逻辑捋一下。
% 第一段，直接图X展示了评估结果（我给你改过了第一句话，直接用就行），说一下方法在三个大维度上的得分情况，然后说比第二名基线数据集高多少。这个地方只讲大维度。
%然后从第二段起，介绍core findings，每个core findings一段话，每段话的第一句剪短写核心的结论（加粗）。第二句话开始写results里面支持的evidence。总体上写2-3个小段就行。
%这2-3个小段，可以从三个维度展开，也可以做一些合并。


% To objectively measure the quality of the training dataset. 
% We evaluate across three dimensions: Planning Reasonableness Score (PRS), Instruction Executability Score (IES), and Intent Consistency Score (IAS).
% Each dimension includes fine-grained sub-dimensions, and the scoring rules are formulated based on the core requirements for the quality of tool training data. 
% PRS focuses on whether the tool selection and execution logic in the data meet the actual task requirements, including \textit{Tool Selection} (the relevance and appropriateness of the selected tools to the target tasks), \textit{Redundancy} (the situation of redundant or unnecessary tool calls in the data; the higher the proportion of redundant calls, the lower the score), and \textit{Execution Order} (the logical coherence of the tool execution sequence in the data; sequences with rigorous logic score higher). IES focuses on whether the tool call instructions in the data comply with the official tool specifications and can be executed correctly, including \textit{Parameter Name} (consistency between parameter names in tool instructions and those in official tool documentation), \textit{Parameter Values} (whether parameter values meet the data type specification of the tool), and \textit{Format Compliance} (whether the parameter transmission format conforms to the specifications of the tool, such as JSON format). IAS focuses on whether the parameter filling in the data accurately consistent with key elements in user queries; when parameters completely match the user queries, a high score is awarded. The Overall quality score is the normalized average of all indicators, used to comprehensively reflect the overall quality of the dataset.

Figure \ref{fig:dataset_quality_dimensions} shows the quality results of the synthetic data, concerting on the dimension and relevant sub-dimension described in Section \ref{sec:experiment_rq1}.
% Final results are shown in Figure~\ref{fig:dataset_quality_dimensions}. 
It can be seen that the dataset generated by our method achieves an overall quality score (a composite metric calculated by averaging the normalized scores of PRS, IES, and IAS) of 0.9758, which is 18.8\% higher than the ToolBench dataset. 
Notably, our dataset performs excellently in all three core dimensions: the normalized score of PRS reaches 0.9827, IES reaches 0.9840, and IAS reaches 0.9308. 
The balanced and high performance across all dimensions indicates that our method can generate tool training data with comprehensive quality advantages.
Furthermore, to ensure the alignment between LLM evaluation results and human, we randomly selected 20\% of the evaluated samples for manual verification. 

Each sample was independently scored by two domain experts, with cross-validation implemented to mitigate subjective bias and enhance reliability. The consistency rate between LLM-generated scores and human expert ratings across all sub-dimensions reached 97.3\%, which fully validates the effectiveness of the LLM-as-a-judge evaluation results.
\yang{comment.}
%这个地方的逻辑是：所有图中展示的结果，都是LLM评出来的？然后人为了确认评估结果的准确性，看了一下llm评估的结果准不准，算了个一致性？
%如果是这样的话，4.1那个要明确一下，先说基础结果是主流的LLM评估出来的，人加以确认。
%这个地方能够改成全部人评估就更好了。

\yang{REV}
% The core reason for these excellent results lies in the data generation strategy we proposed, which systematically ensures the rationality, executability, and intent consistency of the generated data: we first construct executable tool instructions, then have users query based on these pre-set tool instructions to generate data in reverse, ensuring that tool selection is precisely matched with task requirements. 
% Meanwhile, tool trajectories are synthesized according to real business logic to avoid redundancy and logical confusion. Generate in reverse through the parameter center to further enhance the consistency between parameters and user intent. In contrast, baseline methods not only tend to include redundant and irrelevant tool invocations but also suffer from the problem of parameters failing to accurately match user queries.
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{images/dataset_evaluate.pdf} 
    \caption{Results of quality evaluation of the synthetic data} 
    % The radar chart compares TAIA (Ours) against five baselines across four hierarchical dimensions: Planning Rationality (PRS), Instruction Executability (IES), Intent Alignment (IAS), and Query Quality.
    \label{fig:dataset_quality_dimensions}
\end{figure}
% 1. 图太大了，size整体上缩小一点；
% 2. 图上的文字数值太小，正常看看不清楚，字号放大点，看看有没有必要加粗让字更清楚一点；
% 3. 图的单位不统一，有些事%，有些是1，应该是有错误；
% 4. 图现在只有sub-deminsion，突出一下dimension到sub-deminson的对应关系。


% \yang{comment.}
%这一个章节重新按照以下思路梳理一下
% 1. 因为我吧experiment如何进行人工评估介绍删了，第一段先介绍依据4.2.1提出的三个维度，是如何进行打分的，包括你前面提到的人工评估和llm as judge的方法是如何进行的，打分的依据是什么，overall是是什么含义，都简单介绍一下。有一些内容（比如judge的prompt、打分依据）如果正文没有办法详细展开，引导附录里面去；
% 2.总体说一下overall的性能达到最优，比基线高出的百分比是多少。
% 3. 从PRS、IES、IAS三个维度分析，我们的方法具体好在哪里了，可以举具体的例子，阐述为什么我们的方法能够更好的解决。
% \yang{comment.}
%另外这个表现在有点丑，不如吧这个表换成雷达图，下面雷达图换成一个比较详尽的表。
%还有一个点，就是现在这3个维度，其实粒度都比较粗，从前面的4.2.1的内涵来看，表达的内涵也是多层的。这里评估的维度能不能再3个大维度下设置一些更细致的。比如PRS分为工具选择合理性得分，工具链上下游合理性得分；IES先面在细分为参数名有效性得分、参数值有效性得分、格式有效性得分之类的。类似这种在3个大的维度下还能更细一步得拆，这样感觉实验才比较充分。



\subsection{Results of Intent Alignment (RQ2)}
\yang{comment.}
%这个地方好像还是没改够来呢：把IN的评估和你现在table 2的评估结合合到一张表里面去。相当于这种表能看到你两阶段训练的效果提升，也可能看到其他基线方法的性能对比。

We conduct a comprehensive evaluation of the proposed method on five mainstream open-source large language models, with a focus on verifying the role of the obtained data in parameter intent alignment. 
The main results are shown in Table~\ref{tab:model_performance}, where we compare the performance of the original model (Raw), the model using only supervised fine-tuning (SFT) data, the model using only preference data (DPO), and the model optimized with full data based on a two-stage training paradigm (RISE). 
The results show that using our method significantly improves the model's tool usage performance and effectively enhances the performance of key parameter settings.

The OverallAcc of Llama-3.1-8B-Instruct increased from 54.84\% to 83.91\% (+29.07 percentage points), and that of Qwen2.5-7B-Instruct increased from 58.10\% to 82.70\% (+24.60 percentage points). Notably, the initially poorly performing deepseek-llm-7b-chat also achieved a 47.01 percentage point improvement. This verifies that the method can effectively calibrate the model's tool calling capability. Additionally, the IntentAlign rates of all original models were at very low levels, with the IntentAlign scores of open-source tool-enhanced agents in other studies also being very low. As shown in Figure~\ref{fig:baselines}, ToolLLaMA-2-7b-v2 scored only 0.0175, Lynx-7b scored 0.0963, and even the best baseline model ToolAlpaca-7B scored only 0.3268, indicating that existing models have capability deficiencies in parameter-intention mapping and highlighting the limitations of focusing solely on effective tool calling. Our method achieved significant improvements in the IntentAlign metrics of all models, with Llama-3.1-8B-Instruct reaching 62.19\%. This result exceeds that of the closed-source GPT-5 nano model, indicating that our method can effectively guide models to capture key parameter information.

\subsection{Results of Generalization (RQ3)}
To evaluate the performance of RISE on out-of-distribution (OOD) tools, we assessed all models on the ToolBench and NesTools test dataset, which includes unseen tool interfaces and complex multi-step task or nested tool scenarios. As shown in Figure~\ref{fig:toolbench_ood_performance}, RISE consistently improves tool usage performance across various model architectures on the ToolBench dataset. The API accuracy of the Llama-3.1-8B-Instruct model increases from 47.64\% of the original model to 62.09\%, and Mistral-7B rises from an initial 20.10\% to 44.41\%. In terms of task completion, the task accuracy of Llama-3.1-8B-Instruct doubles from 24.00\% to 48\%, and deepseek-llm-7b-chat surges from 7\% to 54\%. The significant improvement in task completion rate indicates that the RISE model focuses more on task-level effectiveness rather than merely following surface-level API formats. The results confirm that RISE can still effectively enhance a model's tool usage capability when faced with unseen tool scenarios. Figure~\ref{fig:nestools_average} shows the average results of multiple precision metrics used in the NesTools benchmark for complex nested tool scenarios, which also verifies RISE's generalization capability on OOD tools.


% \begin{table}[t]
%     \centering
%     \caption{Quality evaluation results of different tool-learning datasets (higher values indicate better quality). All scores are normalized to the range of 0–1 (PRS/IES/IAS normalized by full score 5, overall score normalized by full score 15).}
%     \label{tab:dataset_quality}
%     \setlength{\tabcolsep}{6pt}
%     \small
%     \begin{tabular}{lccccc}
%         \toprule
%         Dataset & Overall & PRS & IES & IAS \\
%         \midrule
%         ToolBench & 0.7190 & 0.7477 & 0.6412 & 0.7682 \\
%         ToolAlpaca & 0.7670 & 0.7917 & 0.7199 & 0.7893 \\
%         STE & 0.7139 & 0.7236 & 0.6934 & 0.7248 \\
%         GPT4Tools & 0.8549 & 0.8108 & \textbf{0.9094} & 0.8446 \\
%         PEToolBench & \textbf{0.9193} & 0.8958 & \textbf{0.9251} & \textbf{0.9369} \\
%         TAIA(Ours) & \textbf{0.9273} & \textbf{0.9362} & \textbf{0.9149} & \textbf{0.9308} \\
%         \bottomrule
%     \end{tabular}
% \end{table}

\begin{table*}[!ht]
    \centering
    % \small
    \caption{The overall tool-using performance on RISE test dataset}
    \label{tab:model_performance}
    \resizebox{\linewidth}{!}{% 自适应页面宽度
        \begin{tabular}{lccccc}
            \toprule[1pt]
            Model & OverallAcc & TaskAcc & APIValid & IntentAlign & F1 Score  \\
            \midrule[0.75pt]
            % Llama-3.1-8B-Instruct 系列
            Llama-3.1-8B-Instruct(Raw) & 54.84\% & 65.60\% & 62.09\% & 37.05\% & 54.63\%  \\
            Llama-3.1-8B-Instruct(SFT) & 76.74\% & 88.58\% & 98.33\% & 60.02\% & 60.02\%  \\
            Llama-3.1-8B-Instruct(DPO) & 56.02\% & 68.83\% & 63.08\% & 38.64\% & 53.51\%  \\
            Llama-3.1-8B-Instruct(\textbf{Ours,RISE}) & \textbf{\underline{83.91\%}} &\textbf{\underline{ 91.98\%}} & \textbf{\underline{98.81\%}} & \textbf{\underline{62.19\%}} & \textbf{\underline{82.66\%}}  \\
            \midrule[0.5pt]
            % Qwen2.5-7B-Instruct 系列
            Qwen2.5-7B-Instruct (Raw) & 58.10\% & 60.03\% & 62.73\% & 48.33\% & 61.30\%  \\
            Qwen2.5-7B-Instruct (SFT) & 81.92\% & 92.28\% & 97.70\% & 55.98\% & 81.70\%  \\
            Qwen2.5-7B-Instruct (DPO) & 57.45\% & 58.49\% & 61.92\% & 49.68\% & 59.70\%  \\
            Qwen2.5-7B-Instruct (\textbf{Ours,RISE}) & \textbf{\underline{82.70\%}} & \textbf{\underline{92.29\%}} & \textbf{\underline{97.84\%}} & \textbf{\underline{58.24\%}} & \textbf{\underline{82.42\%}}  \\
            \midrule[0.5pt]
            % deepseek-llm-7b-chat 系列
            deepseek-llm-7b-chat (Raw) & 27.29\% & 47.84\% & 24.65\% & 17.45\% & 19.20\%  \\
            deepseek-llm-7b-chat (SFT) & 73.62\% & 89.81\% & 81.28\% & 48.43\% & 74.94\%  \\
            deepseek-llm-7b-chat (DPO) & 26.82\% & 50.93\% & 21.44\% & 20.85\% & 14.04\%  \\
            deepseek-llm-7b-chat (\textbf{Ours,RISE}) & \textbf{\underline{74.30\%}} & \textbf{\underline{89.93\%}} & \textbf{\underline{81.24\%}} & \textbf{\underline{50.86\%}} & \textbf{\underline{75.15\%}}  \\
            \midrule[0.5pt]
            % Qwen3-8B 系列
            Qwen3-8B(Raw) & 55.01\% & 67.59\% & 60.77\% & 37.05\% & 54.63\%  \\
            Qwen3-8B(SFT) & 78.43\% & 88.58\% & 83.68\% & 58.88\% & 82.59\%  \\
            Qwen3-8B (DPO) & 57.56\% & 65.90\% & 63.34\% & 47.06\% & 53.94\%  \\
            Qwen3-8B(\textbf{Ours,RISE}) & \textbf{\underline{82.06\%}} & \textbf{\underline{90.90\%}} & \textbf{\underline{95.11\%}} & \textbf{\underline{58.99\%}} & \textbf{\underline{83.24\%}}  \\
            \midrule[0.5pt]
            % Mistral-7B 系列
            Mistral-7B(Raw) & 57.71\% & 70.83\% & 71.32\% & 36.47\% & 52.21\%  \\
            Mistral-7B(SFT) & 64.84\% & 83.03\% & 72.90\% & 45.55\% & 57.89\%  \\
            Mistral-7B(DPO) & 56.85\% & 69.75\% & 69.90\% & 35.84\% & 51.91\% \\
            Mistral-7B(\textbf{Ours,RISE}) & \textbf{\underline{68.22\%}} & \textbf{\underline{83.18\%}} & \textbf{\underline{73.41\%}} & \textbf{\underline{46.79\%}} & \textbf{\underline{69.50\%}}  \\
            \midrule[0.5pt]
ToolLLaMA-2-7b-v2 & 31.69\% & 6.35\% & 94.26\% & 1.75\% & 24.41\%  \\
Lynx-7b & 40.89\% & 41.27\% & 63.94\% & 9.63\% & 48.72\%  \\
ToolAlpaca-7B & 61.18\% & 87.38\% & 72.31\% & 32.68\% & 52.35\%  \\
GPT-5-nano & 70.77\% & 68.99\% & 92.94\% & 57.13\% & 64.00\%  \\
            \bottomrule[1pt]

        \end{tabular}
    }
    \vspace{5pt}
    
\end{table*}

% \begin{table*}[!ht]
%     \centering
%     \caption{The overall tool-using performance on TAIA test dataset}
%     \label{tab:model_performance}
%     \resizebox{0.98\textwidth}{!}{% 适配页面宽度
%         \begin{tabular}{lccccc}
%             \toprule[1pt]
%             \textbf{Model} & \textbf{OverallAcc} & \textbf{TaskAcc} & \textbf{APIValid} & \textbf{IntentAlign} & \textbf{F1 Score}  \\
%             \midrule\midrule
%             % Baselines 部分
%             ToolLLaMA-2-7b-v2 & 31.69\% & 6.35\% & 94.26\% & 1.75\% & 24.41\%  \\
%             Lynx-7b & 40.89\% & 41.27\% & 63.94\% & 9.63\% & 48.72\%  \\
%             ToolAlpaca-7B & 61.18\% & 87.38\% & 72.31\% & 32.68\% & 52.35\%  \\
%             GPT-5-nano & 70.77\% & 68.99\% & 92.94\% & 57.13\% & 64.00\%  \\
%            \midrule\midrule
%             % Llama-3.1-8B-Instruct 系列（按指定样式）
%             Llama-3.1-8B-Instruct & 54.84\% & 65.60\% & 62.09\% & 37.05\% & 54.63\%  \\
%             TAIA-Llama-3.1-8B-Instruct & \underline{\textbf{83.91\%}}\gain{13.14} & \underline{\textbf{91.98\%}}\gain{22.99} & \underline{\textbf{98.81\%}}\gain{5.87} & \underline{\textbf{62.19\%}}\gain{5.06} & \underline{\textbf{82.66\%}}\gain{18.66}  \\
%             w/o DPO & 76.74\% & 88.58\% & 98.33\% & 60.02\% & 60.02\%  \\
%             w/o SFT & 56.02\% & 68.83\% & 63.08\% & 38.64\% & 53.51\%  \\
%             \midrule[0.75pt]
%             % Qwen2.5-7B-Instruct 系列（按指定样式）
%             Qwen2.5-7B-Instruct & 58.10\% & 60.03\% & 62.73\% & 48.33\% & 61.30\%  \\
%             TAIA-Qwen2.5-7B-Instruct & \underline{\textbf{82.70\%}}\gain{11.93} & \underline{\textbf{92.29\%}}\gain{23.30} & \underline{\textbf{97.84\%}}\gain{4.90} & \underline{\textbf{58.24\%}}\gain{1.11} & \underline{\textbf{82.42\%}}\gain{18.42}  \\
%             w/o DPO & 57.45\% & 58.49\% & 61.92\% & 49.68\% & 59.70\%  \\
%             w/o SFT & 81.92\% & 92.28\% & 97.70\% & 55.98\% & 81.70\%  \\
%             \midrule[0.75pt]
%             % deepseek-llm-7b-chat 系列（按指定样式）
%             deepseek-llm-7b-chat & 27.29\% & 47.84\% & 24.65\% & 17.45\% & 19.20\%  \\
%             TAIA-deepseek-llm-7b-chat & \underline{\textbf{74.30\%}}\gain{3.53} & \underline{\textbf{89.93\%}}\gain{20.94} & \underline{\textbf{81.24\%}} & \underline{\textbf{50.86\%}} & \underline{\textbf{75.15\%}}\gain{11.15}  \\
%             w/o DPO & 26.82\% & 50.93\% & 21.44\% & 20.85\% & 14.04\%  \\
%             w/o SFT & 73.62\% & 89.81\% & 81.28\% & 48.43\% & 74.94\%  \\
%             \midrule[0.75pt]
%             % Qwen3-8B 系列（按指定样式）
%             Qwen3-8B & 55.01\% & 67.59\% & 60.77\% & 37.05\% & 54.63\%  \\
%             TAIA-Qwen3-8B & \underline{\textbf{82.06\%}}\gain{11.29} & \underline{\textbf{90.90\%}}\gain{21.91} & \underline{\textbf{95.11\%}}\gain{2.17} & \underline{\textbf{58.99\%}}\gain{1.86} & \underline{\textbf{83.24\%}}\gain{19.24}  \\
%             w/o DPO & 57.56\% & 65.90\% & 63.34\% & 47.06\% & 53.94\%  \\
%             w/o SFT & 78.43\% & 88.58\% & 83.68\% & 58.88\% & 82.59\%  \\
%             \midrule[0.75pt]
%             % Mistral-7B 系列（按指定样式）
%             Mistral-7B & 57.71\% & 70.83\% & 71.32\% & 36.47\% & 52.21\%  \\
%             TAIA-Mistral-7B & \underline{\textbf{68.22\%}}\gain{-2.55} & \underline{\textbf{83.18\%}}\gain{14.19} & \underline{\textbf{73.41\%}} & \underline{\textbf{46.79\%}} & \underline{\textbf{69.50\%}}\gain{5.50}  \\
%             w/o DPO & 56.85\% & 69.75\% & 69.90\% & 35.84\% & 51.91\%  \\
%             w/o SFT & 64.84\% & 83.03\% & 72.90\% & 45.55\% & 57.89\%  \\
%             \bottomrule[1pt]
%         \end{tabular}
%     }
%     \vspace{-10pt} 
% \end{table*}
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1\linewidth]{latex/images/baselines.pdf}
%     \caption{Performance comparison between TAIA model and baseline tool-learning models(ToolLLaMA-2-7b-v2, Lynx-7b, ToolAlpaca-7B).TAIA outperforms all baselines significantly, especially in IntentAlign, highlighting the inadequacy of existing methods in capturing user intent for critical parameters and their poor adaptability to MCP-compliant tools.}
%     \label{fig:baselines}
% \end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{images/toolbench.pdf}
    \caption{Performance comparison of the original model and the RISE model on the out-of-distribution ToolBench dataset.}
    \label{fig:toolbench_ood_performance}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{images/nestools_average.pdf}
    \caption{Average precision comparison of raw models and RISE models on NesTools dataset.}
    \label{fig:nestools_average}
\end{figure}


\subsection{Further Analysis}
To gain a deeper understanding of the effectiveness of our method, we conducted a further analysis of the two-stage training paradigm and the role of the ICP in intention alignment.
\paragraph{Synergistic Value of the Two-Stage Training Paradigm}
The DPO phase in RISE employs parameter preferences guided by ICP to optimize fine-grained intent alignment, addressing the limitation of SFT's insufficient optimization at the parameter-level intent understanding. 
However, we found that training solely on fine-grained preference samples based on parameter variations yields poor performance ((e.g., the OverallACC of Qwen2.5-7B-Instruct(DPO) is only 57.45\%). 
Such data only reflect subtle differences in parameter configurations without prior calibration from SFT, leaving the model lacking the fundamental ability to effectively use tools. This is why standalone DPO cannot bring meaningful improvements. Only when combined with SFT's basic tool usage capability training can the preference learning in the DPO phase fully exert its effect, thereby achieving collaborative optimization.
\paragraph{Critical Role of ICP in Intent Alignment}
The value of ICP determines whether the tool call meet user needs. Unlike required parameters centered on tools, ICP prioritizes task constraints. Existing tool-learning models lack targeted intent-parameter mapping, as their training ignores this intent-centric parameter prioritization. However, the division of ICP clearly guides the data generation process, enabling the LLM's tool using to move toward a deeper level of understanding. This translates to consistent IntentAlign metric improvements: Llama-3.1-8B-Instruct increased from 60.02\% with SFT to 62.19\% with RISE, while that of deepseek-llm-7b-chat increased from 48.43\% with SFT to 50.86\% with RISE.

